Online No-regret Model-Based Meta RL for Personalized Navigation

The interaction between a vehicle navigation system and the driver of the vehicle can be formulated as a model-based reinforcement learning problem, where the navigation systems (agent) must quickly adapt to the characteristics of the driver (environmental dynamics) to provide the best sequence of turn-by-turn driving instructions. Most modern day navigation systems (e.g, Google maps, Waze, Garmin) are not designed to personalize their low-level interactions for individual users across a wide range of driving styles (e.g., vehicle type, reaction time, level of expertise). Towards the development of personalized navigation systems that adapt to a variety of driving styles, we propose an online no-regret model-based RL method that quickly conforms to the dynamics of the current user. As the user interacts with it, the navigation system quickly builds a user-specific model, from which navigation commands are optimized using model predictive control. By personalizing the policy in this way, our method is able to give well-timed driving instructions that match the user's dynamics. Our theoretical analysis shows that our method is a no-regret algorithm and we provide the convergence rate in the agnostic setting. Our empirical analysis with 60+ hours of real-world user data using a driving simulator shows that our method can reduce the number of collisions by more than 60%.

==> analysis.tex <==
% !TEX root =  main.tex 

\section{Analysis}
\label{sec:analysis}

In this section we provide the regret analysis for Alg.~\ref{alg:alg_box}. At a high level, our regret analysis is based on the previous analysis of the online SystemID framework \cite{ross2012agnostic} that applies DAgger \cite{ross2011reduction} in the MBRL setting to train the sequence of models, where DAgger can be regarded as a no-regret online learning procedure such as Follow-the-Leader (FTL) algorithm \cite{shalev2011online}. In our setting, on the other hand, our model training framework could be regarded as Follow-the-Meta-Leader (FTML) \cite{finn2019online} that is also no-regret with our designed training objective. The overall intuition is that with the sequence of more reliable adapted models, the regret can be bounded and diminish over time. We first introduce our assumptions:
\begin{assum}[Optimal Control Oracle]
We assume that the model predictive control methods return us an $\epsilon-\text{optimal}$ policy. That is, for any transitional dynamics kernel $P$ and initial state distribution $\mu$, we have
\[\EE_{s \sim \mu} \left[ V^{P,\text{MPC}(P)}(s) \right] - \min_{\pi \in \Pi} \EE_{s \sim \mu} \left[ V^{P,\pi}(s) \right] \leq \epsilon_{\text{oc}}. \]
\end{assum}

%This assumption ensures that the model predictive control methods could return a policy that incurs low cumulative costs. 
%Note that the $\epsilon_{\text{oc}}$ term is independent of our algorithm (i.e., we can not eliminate this term no matter how carefully we design our algorithm).

\begin{assum}[Agnostic]
We assume agnostic setting. That is, our model class may not contain the ground truth meta model that can perfectly adapt to any dynamics. Formally, given arbitrary state-action distribution $d$, one trajectory $\tau$ induced by $P^{(t)}$, $\exists \widehat{P}^\ast \in \mathcal{P}$, such that $\forall t \in [T]$,
\[\EE_{s,a \sim d} \left[D_{KL}(U(\widehat{P}^\ast, \tau)(\cdot|s,a), P^{(t)}(\cdot|s,a)) \right] \leq \epsilon_{model}.\]
\label{assump:model}
\end{assum}
%Since we are in the meta learning regime, imposing the realizability assumption (i.e., there exists a meta model that can perfectly adapt to any dynamics) would be an overly strong assumption. Instead, the above assumption states that, although we don't assume the existence of the perfect meta model, the KL divergence between the adapted best meta model and the ground truth dynamics is bounded by a small offset for all incoming MDPs. Similar to $\epsilon_{\text{oc}}$, this generalization error $\epsilon_{\text{model}}$ is also algorithm-independent.
Note that $\epsilon_{\text{oc}}$ and $\epsilon_{\text{model}}$ are independent from our algorithm (i.e., we can not eliminate this term no matter how carefully we design our algorithm).


%\begin{assum}[Bounded cost function]
%We assume that the cost function is bounded, i.e., $\forall s \in \Scal, a \in \Acal$,
%\[0 \leq c(s,a) \leq 1.\]
%\end{assum}

Our analysis begins with bounding the performance difference between the sequence of policies generated by our algorithm and any policy $\pi'$, which can be the policy induced by adapting from the best meta-model. As the first step, the following lemma relates the performance difference to the model error. There are two key techniques used in the proof of Lemma~\ref{lemma:perf_model}: 1. we invoke the simulation lemma, which is widely utilized in model-based RL analysis \cite{kearns2002near,sun2019model}, and for completeness we include it in the Appendix. 2. We relate the trajectories induced by $\pi'$ and $\pi^e$ by the coefficient term introduced in the Sec.~\ref{sec:pre}. Note that since we should only care about comparing with ``good" $\pi'$, the coefficient is small under such circumstances.
\begin{lemma}
Let $\{\widehat{P}^{(t)}\}_{t=1}^T$ be the learned meta models. Let $\{U(\widehat{P}^{(t)}, \tau_t)\}_{t=1}^T$ be the adapted model after the one-shot adaptations. Let $\boldsymbol{\widehat{\pi}} = \{\widehat{\pi}^{(t)}\}_{t=1}^T$, where $\widehat{\pi}^{(t)} := MPC(U(\widehat{P}^{(t)}, \tau_t))$. Let $\rho_t := \frac{1}{2}d_{P^{(t)}}^{\widehat{\pi}^{(t)}} + \frac{1}{2}\nu_t$ be the state-action distribution induced by our algorithm under $\Mcal^{(t)}$. Then for policy sequence $\boldsymbol{\pi'} = \{\pi'^{(t)}\}_{t=1}^T$, we have:
\begin{align*}
    J_{\mu}(\boldsymbol{\widehat{\pi}}) - J_{\mu}(\boldsymbol{\pi'})  &\leq {\epsilon}_{oc} +  \frac{2\max_t(c_{\nu_i}^{\pi'^{(t)}})H^2}{T} \sum_{t=1}^{T}  \mathbb{E}_{s,a\sim \rho_t} \|U(\widehat{P}^{(t)}, \tau_t)(\cdot | s,a) 
    - P^{(t)}(\cdot | s,a)\|_1 
\end{align*}
\label{lemma:perf_model}
\end{lemma}
%{\color{blue}{Wen: $\boldsymbol{\pi'}$ is undefined.., and $\max$ is over what? I'm not sure what meta policy means (if you want to use this term in theorems/lemmas, you need to define it VERY clearly...in this lemma, it should hold for any sequence of policies $\boldsymbol{\pi}$? or it needs to be a sequence of policies associated with the best meta model P?}}

The next step is thus to bound the model error over the online process. Let's first observe the following loss function:
$
    \ell^{(t)}(P) = \EE_{s,a \sim \rho_t} \left[D_{KL}\left( P(\cdot|s,a), P^{(t)}(\cdot|s,a) \right) \right], 
$
where $\rho_t$ defined as in Lemma~\ref{lemma:perf_model}, is the state-action distribution of our data collection scheme. Then if we use FTML to update the meta model:
$
    \widehat{P}^{(t+1)} = \argmin_{P \in \Pcal} \sum_{i=1}^t \ell^{(t)}(U(P, \tau_t)),
$
it is easy to see this update is equivalent to Eq.~\ref{eq:ftml} as in our algorithm. Then we can invoke the main result from \cite{finn2019online} (we restate in Lemma~\ref{lemma:ftml} for completeness), and combine the above lemmas and assumptions, we are ready to present our main result:
%{\color{blue}{Wen: define $\boldsymbol\pi'$..is $\pi_t'$ in $\boldsymbol\pi'$ the optimal policy of $U(P^\star,\tau_t)$, where $P^\star$ is the best meta model? }}
\begin{theorem}
Following notations in Lemma~\ref{lemma:perf_model}, we have \footnote{Note that $\Tilde{O}$ hides the logarithmic terms.}:
\begin{align*}
     J_{\mu}(\boldsymbol{\widehat{\pi}}) - J_{\mu}(\boldsymbol{\pi'})  \leq \epsilon_{oc} + \max_t(c_{\nu_t}^{\pi'^{(t)}})H^2 \sqrt{\epsilon_{\text{model}}} 
+\Tilde{O}\left( \frac{\max(c_{\nu_t}^{\pi'^{(t)}}) H^2}{\sqrt{T}} \right)
\end{align*}
\label{thm:main}
\end{theorem}
%{\color{blue}{Why this is $1/\sqrt{T}$? you were using $\log(T)$ rate in FTRL?}}
We defer the full proofs in Appendix~\ref{app:proofs}. Thm.~\ref{thm:main} shows that given any $\boldsymbol{\pi'}$, which could be the policies induced by the best meta model in the model class, the performance gap incurred by our algorithm diminishes with rate $\Tilde{O}(\frac{1}{\sqrt{T}})$, along with the inevitable terms $\epsilon_{\text{oc}}$ and $\epsilon_{\text{model}}$, which our algorithm has no control over. Since our main result is based on any arbitrary policy sequence, we here first formally define the best adapted sequence of policies from hindsight, and we could easily conclude with the no-regret conclusion in the following corollary:
\begin{corollary}
Let $\boldsymbol{\widehat{\pi}} = \{\widehat{\pi}^{(t)}\}_{t=1}^T$ be the policies returned by our algorithm. Define $\pi^{\ast}_{P} = \argmin_{\pi \in \Pi}\EE_{s \sim \mu}V^{\pi,P}(s)$. Let $\boldsymbol{\pi^{\ast}}_P = \{\pi^{\ast}_{U(P,\tau_t)}\}_{t=1}^T$. For simplicity let $\pi^{\ast(t)} = \pi^{\ast}_{U(P,\tau_t)}$. Let $R(T) = J(\boldsymbol{\widehat{\pi}}) - \min_{P \in \Pcal}J(\boldsymbol{\pi^{\ast}}_P)$ be the regret of our algorithm. We have
\begin{align*}
    \lim_{T \to \infty} R(T) = \epsilon_{oc} +\max_t(c_{\nu_t}^{\pi^{\ast(t)}})H^2 \sqrt{\epsilon_{\text{model}}}.
\end{align*}
\end{corollary}
%Thus if we further assume realizability and a perfect control (i.e., $\epsilon_{\text{oc}} = 0$ and $\epsilon_{\text{model}} = 0$), we obtain that our regret goes to 0 asymptotically.
